LAFEAT: Piercing Through Adversarial Defenses with Latent Features

Deep convolutional neural networks are susceptible to adversarial attacks. They can be easily deceived to give an incorrect output by adding a tiny perturbation to the input. This presents a great challenge in making CNNs robust against such attacks. An influx of new defense techniques have been proposed to this end. In this paper, we show that latent features in certain "robust" models are surprisingly susceptible to adversarial attacks. On top of this, we introduce a unified $\ell_\infty$-norm white-box attack algorithm which harnesses latent features in its gradient descent steps, namely LAFEAT. We show that not only is it computationally much more efficient for successful attacks, but it is also a stronger adversary than the current state-of-the-art across a wide range of defense mechanisms. This suggests that model robustness could be contingent on the effective use of the defender's hidden components, and it should no longer be viewed from a holistic perspective.

==> scratch.tex <==
From a human perception perspective,
it has been known
that as feature extractors,
deeper layers of CNNs
extract increasingly higher-level features
\cite{olah17feature,carter19activation},
\ie~shallow layers
extract simple local textures
while neurons in deep layers
specialize to differentiate complex objects.


\begin{equation}
    \begin{aligned}
    & \max_{\mathclap{
        \logit{1:N},\,
        \logitweight{1:N},\,
        \alpha_{0:T},\,
        \surrogateloss
    }}
    \sceloss\left(
        f_\allw\left( \xadv \right), \y
    \right) \\
    \textit{s.t.} \quad
    \xadv_{0} &= \project (\x + \mathrm{u}),
    \mathrm{u} \sim \uniform{[-\epsilon, \epsilon]} \\
    \bm{o}_t &=
        {\textstyle\sum_{l \in [1:N]}}
        \lambda_{l} \logit{l} \left(
            \idx\xadv{l}_t
        \right), \\
    \xadv_{t+1} &= \project \left(
        \xadv_{t} + \alpha_{t} \sign\left(
            \nabla_{\xadv_t}
            \surrogateloss\left(
                \bm{o}_t,
                \y
            \right)
        \right)
    \right),
    \end{aligned}\label{eq:latent}
\end{equation}


==> tables/16way_ablation.tex <==
\begin{table*}[ht]
\scriptsize
\begin{tabular}{@{}llllllllllllllllll@{}}
      &        &     &        & 32    & 30    & 29    & 26    & 24    & 23    & 21    & 18    & 9     & 8     & 5     & 3     & 2     & 1     \\
      &        &     &        & 13.42 & 0.28  & 1.35  & 34.22 & 36.45 & 36.64 & 40.22 & 43.41 & 53.08 & 53.33 & 54.90 & 56.29 & 57.14 & 59.53 \\
      &        &     &        & 78.16 & 19.01 & 75.72 & 59.88 & 73.13 & 68.82 & 79.75 & 46.26 & 55.48 & 56.48 & 57.54 & 62.20 & 59.84 & 62.09 \\
scale &        &     &        & 78.21 & 20.08 & 75.41 & 62.63 & 73.17 & 68.98 & 40.39 & 44.03 & 53.42 & 53.69 & 55.28 & 57.37 & 57.52 & 60.01 \\
      & linear &     &        & 68.13 & 8.11  & 52.78 & 56.57 & 71.45 & 64.41 & 79.75 & 45.99 & 55.25 & 56.30 & 57.17 & 61.70 & 59.57 & 61.70 \\
scale & linear &     &        & 68.17 & 8.54  & 52.48 & 59.10 & 71.51 & 64.41 & 40.13 & 43.87 & 53.28 & 53.52 & 55.14 & 56.92 & 57.42 & 59.75 \\
      &        & pre &        & 12.73 & 0.38  & 0.48  & 35.09 & 36.40 & 37.22 & 74.89 & 45.85 & 55.13 & 56.02 & 56.73 & 61.20 & 59.48 & 61.79 \\
scale &        & pre &        & 12.59 & 0.44  & 0.42  & 34.66 & 36.27 & 36.90 & 40.26 & 43.83 & 53.26 & 53.49 & 55.16 & 56.90 & 57.37 & 59.80 \\
      & linear & pre &        & 11.97 & 0.09  & 0.35  & 34.44 & 35.91 & 36.58 & 74.89 & 45.6  & 54.96 & 55.83 & 55.61 & 60.99 & 59.27 & 61.48 \\
scale & linear & pre &        & 11.93 & 0.12  & 0.34  & 34.04 & 35.76 & 36.39 & 39.99 & 43.68 & 53.10 & 53.32 & 55.0  & 56.74 & 57.20 & 59.60 \\
      &        &     & target & 35.60 & 10.61 & 15.72 & 45.65 & 52.80 & 39.78 & 40.17 & 44.37 & 53.74 & 54.67 & 55.74 & 58.44 & 58.07 & 60.43 \\
scale &        &     & target & 22.88 & 7.47  & 17.27 & 37.92 & 44.30 & 38.59 & 40.08 & 43.55 & 53.22 & 53.43 & 55.04 & 56.59 & 57.30 & 59.71 \\
      & linear &     & target & 27.24 & 3.36  & 6.19  & 41.84 & 49.72 & 38.25 & 39.92 & 44.28 & 53.65 & 54.54 & 55.66 & 58.17 & 57.91 & 60.27 \\
scale & linear &     & target & 18.27 & 2.12  & 6.64  & 36.55 & 41.43 & 37.33 & 39.88 & 43.40 & 53.07 & 53.28 & 54.84 & 56.28 & 57.15 & 59.52 \\
      &        & pre & target & 11.44 & 0.16  & 0.27  & 33.72 & 35.73 & 36.35 & 40.08 & 44.32 & 53.65 & 54.45 & 55.54 & 58.02 & 57.92 & 60.35 \\
scale &        & pre & target & 11.47 & 0.19  & 0.26  & 33.98 & 35.71 & 36.39 & 39.93 & 43.46 & 53.16 & 53.33 & 54.96 & 56.34 & 57.24 & 59.62 \\
      & linear & pre & target & 11.20 & 0.04  & 0.22  & 33.38 & 35.32 & 36.04 & 39.86 & 44.22 & 53.55 & 53.40 & 55.49 & 57.84 & 57.78 & 60.21 \\
scale & linear & pre & target & 11.18 & 0.06  & 0.23  & 33.59 & 35.31 & 36.06 & 39.81 & 43.33 & 53.02 & 53.22 & 54.80 & 56.15 & 57.08 & 59.43
\end{tabular}
\end{table*}


==> tables/trades.tex <==
\begin{table}[ht]
\centering
\caption{%
    The TRADES~\cite{zhang19trades}
    \cifarx{} white-box leaderboard.
}\label{tab:trades}
\begin{tabular}{lc}
    \toprule
    \textbf{TRADES~leaderboard} & \textbf{Accuracy (\%)} \\
    \midrule
    Nominal~\cite{zhang19trades} & 56.43 \\
    MT~\cite{gowal19surrogate} & 53.07 \\
    FAB~\cite{croce20fab} & 53.44 \\
    AA~\cite{croce20aa} & 53.08 \\
    ODI-PGD~\cite{tashiro2020ods} & 53.01 \\
    EWR-PGD~\cite{ewrpgd} & 52.95 \\
    \midrule
    \att{MT}{1000} & \textbf{52.94} \\
    \bottomrule
\end{tabular}%
\vspace{-10pt}%
\end{table}%

